On the geometric convergence for MALA under verifiable conditions

While the Metropolis Adjusted Langevin Algorithm (MALA) is a popular and widely used Markov chain Monte Carlo method, very few papers derive conditions that ensure its convergence. In particular, to the authors' knowledge, assumptions that are both easy to verify and guarantee geometric convergence, are still missing. In this work, we establish $V$-uniformly geometric convergence for MALA under mild assumptions about the target distribution. Unlike previous work, we only consider tail and smoothness conditions for the potential associated with the target distribution. These conditions are quite common in the MCMC literature and are easy to verify in practice. Finally, we pay special attention to the dependence of the bounds we derive on the step size of the Euler-Maruyama discretization, which corresponds to the proposal Markov kernel of MALA.

==> header.tex <==
% \makeatletter
% %\renewcommand{\algocf@captiontext}[2]{#1\algocf@typo. \AlCapFnt{}#2} % text of caption
% \renewcommand{\AlTitleFnt}[1]{#1\unskip}% default definition
% \def\@algocf@capt@plain{top}
% \renewcommand{\algocf@makecaption}[2]{%
%   \addtolength{\hsize}{\algomargin}%
%   \sbox\@tempboxa{\algocf@captiontext{#1}{#2}}%
%   \ifdim\wd\@tempboxa >\hsize%     % if caption is longer than a line
%     \hskip .5\algomargin%
%     \parbox[t]{\hsize}{\algocf@captiontext{#1}{#2}}% then caption is not centered
%   \else%
%     \global\@minipagefalse%
%     \hbox to\hsize{\box\@tempboxa}% else caption is centered
%   \fi%
%   \addtolength{\hsize}{-\algomargin}%
% }
% \makeatother

%%% fix for miktex
\makeatletter
\def\set@curr@file#1{%
  \begingroup
    \escapechar\m@ne
    \xdef\@curr@file{\expandafter\string\csname #1\endcsname}%
  \endgroup
}
\def\quote@name#1{"\quote@@name#1\@gobble""}
\def\quote@@name#1"{#1\quote@@name}
\def\unquote@name#1{\quote@@name#1\@gobble"}
\makeatother
\usepackage{graphics}


%\documentclass[11pt]{article}

%\usepackage[a4paper]{geometry} % required for statsoc+pdflatex


% \usepackage[notref,notcite]{showkeys}  %  comment out for final version
% \renewcommand*\showkeyslabelformat[1]{\fbox{\normalfont\scriptsize\sffamily#1}}   % for showkeys
%\usepackage{showframe}

\usepackage[utf8]{inputenc}
\usepackage{amssymb}
\usepackage{makeidx}
\usepackage[T1]{fontenc}
\usepackage[english]{babel}
\usepackage{graphicx}
\usepackage{graphicx,subcaption}
 \usepackage{amsfonts,amsmath,amssymb}

 % % \usepackage{amsfonts,amsmath}
%\usepackage{epstopdf}
%\usepackage{lmodern}
\usepackage{oldgerm}
%\usepackage{euler}
\usepackage{relsize}

\usepackage{mathrsfs}
\usepackage[active]{srcltx}
\usepackage{verbatim}
\usepackage[shortlabels]{enumitem} %label option for enumerate \alph* \Alph* \roman* \Roman* or other... [label=$\bullet$], [label=\alph*]
%\usepackage[comma,authoryear,longnamesfirst]{natbib}
%\usepackage[backend=biber, style=alphabetic]{biblatex}
%\addbibresource{../bibliography/bibliographie.bib} %% Compiler avec biber
%\usepackage{enumerate}
\usepackage[toc,page]{appendix}
 \usepackage{aliascnt,bbm}
 \usepackage{array}
 % \usepackage[colorlinks = true, citecolor = blue]{hyperref}
%  \usepackage{hyperref}
% %\usepackage[ruled,vlined]{algorithm2e}
\usepackage[textwidth=3cm,textsize=footnotesize]{todonotes}
%\usepackage[disable]{todonotes}
\usepackage{xargs}
\usepackage{cellspace}

%\usepackage{slashbox}
\usepackage[Symbolsmallscale]{upgreek}
%\usepackage{environ}
\usepackage{xstring}
\usepackage{array,multirow,makecell}
\usepackage{booktabs}

%\usepackage[novbox]{pdfsync}           %  [novbox] helps

% For mathematical formula to fit nicely in tables
\usepackage{array,multirow,makecell}
\usepackage{nicefrac}
%\setcellgapes{4pt}
%\makegapedcells
%\newcolumntype{R}[1]{>{\raggedleft\arraybackslash }b{#1}}
%\newcolumntype{L}[1]{>{\raggedright\arraybackslash }b{#1}}
%\newcolumntype{C}[1]{>{\centering\arraybackslash }b{#1}}
%\usepackage{slashbox}

%\usepackage{vmargin} % required for statsoc+pdflatex

\usepackage{natbib}

\usepackage{accents}
\usepackage{dsfont}
\usepackage{aliascnt}
\usepackage{cleveref}
\usepackage{autonum}
\makeatletter
%\newtheorem{theorem}{Theorem}
\crefname{theorem}{theorem}{Theorems}
\Crefname{Theorem}{Theorem}{Theorems}


%\newaliascnt{lemma}{theorem}
%\aliascntresetthe{lemma}
\crefname{lemma}{lemma}{lemmas}
\Crefname{Lemma}{Lemma}{Lemmas}

\crefname{corollary}{corollary}{corollaries}
\Crefname{Corollary}{Corollary}{Corollaries}

\crefname{proposition}{proposition}{propositions}
\Crefname{Proposition}{Proposition}{Propositions}

\crefname{definition}{definition}{definitions}
\Crefname{Definition}{Definition}{Definitions}


\crefname{definition-proposition}{definition-proposition}{definitions-propositions}
\Crefname{Definition-Proposition}{Definition-Proposition}{Definitions-Propositions}

\crefname{remark}{remark}{remarks}
\Crefname{Remark}{Remark}{Remarks}


%\newtheorem{example}[theorem]{Example}
\crefname{example}{example}{examples}
\Crefname{Example}{Example}{Examples}


\crefname{figure}{figure}{figures}
\Crefname{Figure}{Figure}{Figures}

\crefname{table}{table}{tables}
\Crefname{Table}{Table}{Tables}


%\newtheorem{assumptionH}{\textbf{H}\hspace{-4pt}}
%\theoremnumbering{arabic}
\Crefname{assumptionH}{\textbf{H}\hspace{-4pt}}{\textbf{H}\hspace{-4pt}}
\crefname{assumptionH}{\textbf{H}}{\textbf{H}}

\newtheorem{assumptionA}{\textbf{A}\hspace{-4pt}}
\Crefname{assumptionA}{\textbf{A}\hspace{-6pt}}{\textbf{A}\hspace{-6pt}}
\crefname{assumptionA}{\textbf{A}}{\textbf{A}}

\newtheorem{assumptionS}{\textbf{S}\hspace{-3pt}}
\Crefname{assumptionS}{\textbf{S}\hspace{-3pt}}{\textbf{S}\hspace{-3pt}}
\crefname{assumptionS}{\textbf{S}}{\textbf{S}}


\newtheorem{probleme}{\textbf{Problem}}
\Crefname{probleme}{\textbf{Problem}\hspace{-3pt}}{\textbf{Problem}\hspace{-3pt}}
\crefname{probleme}{\textbf{Problem}}{\textbf{Problem}}


\newtheorem{assumptionG}{\textbf{G}\hspace{-4pt}}
\Crefname{assumptionG}{\textbf{G}\hspace{-4pt}}{\textbf{G}\hspace{-4pt}}
\crefname{assumptionG}{\textbf{G}}{\textbf{G}}


% Description environment, to reference to items, like Cref.
% \makeatletter
% \newcommand{\mylabel}[2]{#2\def\@currentlabel{#2}\label{#1}}
% \makeatother

%%%% ANAND %%%%%%%%

%\graphicspath{{figures/}}
%\usepackage{float}

%\usepackage{tikz}


%%% Local Variables:
%%% mode: latex
%%% TeX-master: "main"
%%% End:


==> related_work.tex <==

\paragraph{Comparison with existing litterature}


MALA has been shown to be uniformly geometrically ergodic in \cite{roberts:tweedie:1996} but under very restrictive conditions which we recall. 
Define for any $x \in\rset^d$,
\begin{equation}
  A(x) = \ensemble{y \in\rset^d}{\pi(x)r_{\gamma}(x,y)\leq \pi(y)r_{\gamma}(y,x)} \eqsp, \quad I(x) = \ensemble{y\in\rset^d}{\norm{y} \leq \norm{x}} \eqsp.
\end{equation}
We say that $A$ converges inward in $r_{\gamma}$ for $\gamma >0$ if
\begin{equation}
  \label{eq:1}
  \lim_{\norm{x} \to \plusinfty}\int_{\rset^d} \1_{A(x)\cap I(x)}(y)r_{\gamma}(x,y) \rmd x = 0 \eqsp. 
\end{equation}

Define for any $a \geq 0$, $  \VlyapUnMALA_a(x) = \exp(a \norm{x})$.


\begin{theorem}[\protect{\cite[Theorem 4.1]{roberts:tweedie:1996}}]
  \label{theo:2}
Let $\gamma >0$.  Assume that there exists $\eta >0$ such that 
\begin{equation}
  \label{eq:tail_U}
    \liminf_{\norm{x} \to \plusinfty} \{\norm{x} - \normLigne{x - \gamma \nabla U(x)} \}\geq \eta \eqsp,
  \end{equation}
  and $A$ converges inward in $r_{\gamma}$. Then $\Rmala_{\gamma}$ is $\VlyapUnMALA_{a}$-uniformly geometrically ergodic for $a \in \ooint{0,\gamma \eta}$, \ie, there exist $C_{\gamma} \geq 0$ and $\kappa_{\gamma} >0$ such that 
  for any $x \in \rset^d$,
  \begin{equation}
    \label{eq:2_0}
    \Vnorm[\VlyapUnMALA_{a}]{\updelta_x \Qmala_{\gamma} - \pi} \leq C_{\gamma} \rme^{-\kappa_{\gamma} \gamma k} \VlyapUnMALA_{a}(x) \eqsp. 
  \end{equation}
\end{theorem}

Let us comment \Cref{theo:2}. First, while \eqref{eq:tail_U} is
relatively easy to verify under mild assumptions on the tail of $\pi$,
deriving practical conditions on $U$ ensuring that $A$ converges
inward in $r_{\gamma}$ is very hard and \cite{roberts:tweedie:1996}
only succeeds in showing that this holds in the one-dimensional
setting and under strong conditions on $U$.  Second, 
 \Cref{theo:2} is non quantitative
and therefore the constants in the geometric convergence of $Q_{\gamma}$ to $\pi$ can depend dramatically on the stepsize $\gamma$ which in general has to be chosen small to ensure that a non-negligeable proportion of candidates is accepted during the algorithm. For example, from the optimal scaling for MALA obtained in \cite{roberts:rosenthal:1998} shows that the stepsize should scales as $d^{-1/3}$ as $d \to \plusinfty$ in the ideal scenario where $\pi = \pi_1^{\otimes d}$ for some one-dimensional distribution $\pi_1$. 
Even if these constants would be independent of $\gamma$\footnote{which is not the case in the one-dimensional example considered in \cite{roberts:tweedie:1996} after a careful review of the computation}, we can note that
the parameter $a$ of the Lyapunov function $\VlyapUnMALA_{a}$ has to be
chosen proportional to the stepsize $\gamma$ which implies that the convergence behaves badly with respect to $\gamma$ for unbounded functions. Finally, this result does not provide any recommendation for the choice of $\gamma$ ensuring geometric convergence. 
We aim at addressing all these issues in what follows. In particular, we directly consider the following condition on the potential $U$ in contrast to \cite{roberts:tweedie:1996}.

%%% Local Variables:
%%% mode: latex
%%% TeX-master: "main"
%%% End:

